Using Deep Learning for Morphological Classification in Pigs with a Focus on Sanitary Monitoring

The aim of this paper is to evaluate the use of D-CNN (Deep Convolutional Neural Networks) algorithms to classify pig body conditions in normal or not normal conditions, with a focus on characteristics that are observed in sanitary monitoring, and were used six different algorithms to do this task. The study focused on five pig characteristics, being these caudophagy, ear hematoma, scratches on the body, redness, and natural stains (brown or black). The results of the study showed that D-CNN was effective in classifying deviations in pig body morphologies related to skin characteristics. The evaluation was conducted by analyzing the performance metrics Precision, Recall, and F-score, as well as the statistical analyses ANOVA and the Scott-Knott test. The contribution of this article is characterized by the proposal of using D-CNN networks for morphological classification in pigs, with a focus on characteristics identified in sanitary monitoring. Among the best results, the average Precision metric of 80.6\% to classify caudophagy was achieved for the InceptionResNetV2 network, indicating the potential use of this technology for the proposed task. Additionally, a new image database was created, containing various pig's distinct body characteristics, which can serve as data for future research.

==> Revis__o_Bedin.tex <==
%RESCREVENDO ALGUMAS COISAS COM BASE EM UM OTIMIZADOR APENAS

%PARA "ENXUGAR" O ARTIGO

%Introdução - Copiando o material do Junior

%ABSTRACT

The purpose of this paper is to demonstrate the effectiveness of using D-CNN (Deep Convolutional Neural Networks) for the morphological classification of pigs, with a focus on sanitary monitoring. The study used six different algorithms, including DenseNet201, EfficientNet, InceptionResNetV2, InceptionV3, MobilinetV2, and Xception, and the optimizer Adagrad OR Nadam, OR SGD. The study focused on several pig characteristics, including caudophagy, ear hematoma, scratches on the body, redness, and natural stains (brown or black). The aim of this study is to evaluate the use of D-CNN to monitor the health of pigs, specifically by detecting certain body characteristics that indicate a health deviation. The results of the study showed that D-CNN was effective in detecting deviations related to skin characteristics. However, for body contour characteristics, additional techniques were necessary. Overall, this study contributes to the development of automated systems for monitoring the health of pigs. By using D-CNN and other artificial intelligence techniques, it may be possible to detect health deviations in pigs more quickly and accurately than with traditional methods. This could potentially improve the efficiency and effectiveness of pig farming and contribute to the overall health and well-being of the animals.

%INTRODUÇÃO

Sanitary monitoring in swine farming is a crucial aspect of ensuring the overall health and well-being of the herd, as well as the safety and quality of the pork products produced \cite{Brum2013Doencas}. The concept of sanity monitoring involves regular and systematic monitoring of the health status of the swine herd, with the aim of identifying and addressing any potential health issues or diseases before they become more serious problems. Sanity monitoring typically involves a range of focused inspections and assessments, including monitoring for common symptoms such as sneezing, coughing, diarrhea, omphalitis, and lameness \cite{ABCS2014Produco}.


According to \citet{Barron1952Siwne}, some of the main visual characteristics to consider include the color of the pig's dermis, any scratch marks or cuts, and the presence of abscesses, skin spots, or crusts on the skin. A healthy pig should have a rosy or blushing dermis color, an excessively white or pale dermis color may indicate anemia and reddish tones tending to purple may indicate poor blood circulation or breathing problems. Scratch marks, cuts, and signs of recent cannibalism or aggressive behavior can also indicate health or behavioral issues in pigs. Other visual characteristics such as abscesses, skin spots, and crusts on the skin can also be indicative of health issues in pigs. Overall, regularly monitoring the visual characteristics of pigs is an important aspect of ensuring their health and wellbeing. Identifying and addressing potential health issues early on can help prevent the spread of disease and improve the overall health of the pig herd.


As commented by \cite{Carrion2020Computer}, early detection of diseases can be a critical factor in preventing and controlling outbreaks. Computer vision and machine learning can indeed be powerful tools in epidemiology and disease control. In the context of animal production, computer vision and machine learning can be used to monitor the health and well-being of livestock, allowing farmers and other stakeholders to quickly identify and address any issues that may arise. Overall, the use of computer vision and machine learning in epidemiology and disease control has enormous potential, and there are many exciting research opportunities in this area\cite{Gomez2021ASystematic} \cite{Larsen2021Information}.


The fact that 96\% of publications involving information systems and monitoring sensors applied to swine health and well-being were published between 2016 and 2021 is a strong indication that this is a research field that has been expanding rapidly in recent years \cite{Larsen2021Information}. Among the technologies that are being developed, we can mention load cells, microphones, photoelectric sensors, RFID, thermal cameras, and digital camera applications \cite{Gomez2021ASystematic}.

Digital cameras can indeed be an important tool for monitoring and identifying herd health conditions and well-being in swine \cite{Wurtz2019Recording}. Computer vision and artificial intelligence are tools for obtaining information automatically through digital images and videos. The selection of the right techniques for varied applications can make a big difference in the results of developed algorithm performance and tasks \cite{brunger2020panoptic}, \cite{yang2020review}.

As mentioned by \citet{Madonna2019Precision}, computer vision technology can be used to analyze images or videos of animals and detect abnormalities and other indicators of health problems in swine. Problems like cachexia, lameness, cannibalism injuries, uterine prolapses, rectal, open wounds and scratches are factors that can indicate some symptoms that a possible illness hits the animal. Yet this kind of technology is considered a non-invasive method to measure the health status of the animals.

There are several computational methods listed in the bibliography that can be used to identify pigs, track their posture and behavioral patterns, and assess their health and well-being \cite{Domun2019Learning} \cite{brunger2020panoptic}. The use of vertical illumination and image capture by upper view, using primarily color images (RGB) in 2D is a common approach in many researches \cite{riekert2020automatically}. Overall, the selection of camera positioning and lighting conditions is a critical aspect of any imaging-based research project, and researchers should carefully consider these factors when designing their experiments \cite{yang2020review}.

Deep Convolutional Neural Networks (D-CNNs) are a type of deep learning algorithm that is widely used in computer vision systems and other artificial intelligence applications. They have shown good performance in machine learning tasks such as data processing, image classifications and natural language processing \cite{ALBAWI207Understanding}.

Regarding research using CNN applied in swine, it's possible to list some works that used this architecture. Among them, there is pig facial recognition using D-CNN and high image resolution \cite{MARSOT2020PIGFACE}, and also using the same kind of neural network to identify 10 pig's faces using standard image resolution \cite{HANSEN2018Towards}.

The R-CNN was used by \citet{Tu2021automatic} for making segmentation and automatic detection in pigs. While \citet{XU2022ResearchLying} applied CNN-SVM to image segmentation in pigs to determine the automatic body score of these animals. Another research made by \cite{Witte2021Evaluation} used the Mask-CNN in comparison with other neural networks to compare the metrics in swine segmentation in the production environment.

The behavior of caudophagy was detected using CNN in studies by \cite{liu2020computer} and in studies of caudophagy with diarrhea occurrence by \cite{Domun2019Learning}. Other studies have focused on recognizing feeding behavior \cite{chen2020classification}, monitoring behavior patterns in environments with varying concentrations of greenhouse gases \cite{Anil2021Deep}, using Faster R-CNN and YOLOv4. Additionally, another study used Mask CNN to detect pig mounting behavior \cite{Li2019MountingBehavior}.

Some related works to posture detection in pigs using CNN, being able to quote articles like \cite{ZHU2020AutomaticRecognition} with a focus on sows posture detection using R-CNN in 2D RGB images, and this network could identify postures as standing, seated, lay sideways and belly down.  And the work of \cite{ZHU2020AutomaticRecognition} made the same posture recognition using the same technique. The article published by \cite{XU2022AutomaticScoring} studied patterns of lying down group pigs using CNN-SVM, and how these animals arrange themselves in relation to temperature and were verified that the different postures by the group indicate some productive factors, herd well-being, and health status.

The aim of this paper is to demonstrate the applicability of CNN architectures for classifying morphological characteristics in pig bodies to automate sanitary monitoring in pig farming. The authors used a deep CNN (D-CNN) to classify images of pigs based on morphological characteristics that indicate health deviations, such as caudophagy, ear hematoma, scratches, redness, and natural stains. The authors collected a dataset of pig images and manually labeled them according to the presence or absence of each morphological characteristic. They then used a D-CNN to automatically classify the images based on these characteristics. Overall, this study demonstrates the potential of using CNN architectures for automated sanitary monitoring in pig farming, which can help to improve pig welfare and productivity by enabling early detection and treatment of health deviations.
It's interesting to know that the study evaluated the performance of different CNN architectures, including DenseNet201, EfficientNet, InceptionResNetV2, InceptionV3, MobiliNetV2, and Xception, and used the optimizer SGD or Nadam or Adagrad The use of different architectures and optimizers can have a significant impact on the performance of the CNN models in image classification tasks. By evaluating the performance of multiple architectures and optimizers, the study aims to identify the best combination of architecture and optimizer for the specific task of classifying morphological characteristics in pig bodies. This approach can help to optimize the performance of the CNN models and improve the accuracy of the classification results, which is crucial for the success of automated sanitary monitoring in pig farming.


%MATERIAIS E MÉTODOS

%IMAGE ACQUISITION

%ALGORITHMS
%%% Acho que architectures fica melhor que kinds
%%% Acho que podemos pensar em usar só SGD
To develop this work, six different kinds of D-CNN and ONE optimizer were used for each morphology to be classified. The purpose was to analyze the performance of each network and its optimizer for each morphology classification condition. The networks used were EfficientNet, Xception, DenseNet201, InceptionResNetV2, InceptionV2, and MobilinetV2, and the optimizers used were SGD OR Adagrad OR Nadam.

Regarding the D-CNN networks, EfficientNet is a method of scaling that evenly estimates all dimensions of depth, width, and resolution using a simple yet effective compound coefficient \cite{Tan2020Efficient}. The Xception network is characterized by an intermediate step between regular convolution and depthwise convolution operations, followed by a depthwise convolution and pointwise convolution \cite{Francois_Xception_17}.

The DenseNet201 concept connects all layers in a feed-forward way. For each layer, the feature maps of all previous layers are used as input, and its feature maps are used as input in all subsequent layers \cite{Huang2018Densely}. InceptionResNetV2 uses the empirical concept of training the model using residual connections to significantly accelerate the Inception training step \cite{InceptionResnetV2_2016}.

 Inception-V2 is a convolutional neural network architecture introduced as an improvement over the original Inception architecture. Inception-V2 is based on an inverted residual structure, where the shortcut connections are between the intermediate layers. The idea behind this structure is to use depth-wise convolutions to reduce the number of parameters and then use 1x1 convolutions to increase the depth of the feature maps \cite{InceptionV2_2018}. On the other hand, MobileNetV3 is another convolutional neural network architecture specifically designed for mobile devices, such as smartphones. It was developed using a combination of network hardware architecture (NAS) and the NetAdapt algorithm. The NAS approach involves the use of reinforcement learning to search for optimal neural network architectures, while NetAdapt is an algorithm used to adapt neural networks to different hardware constraints \cite{MobileNetV3}.

%ABOUT OPTMIZERS USAR O PARAGRAFO DE BAIXO OU OS PROXIMOS - DEIXEI DESTACADO
 In relation to optimizers, The SGD algorithm works on the principle that when the momentum stochastic descent gradient uses a well-done random initialization for the momentum parameter, it can train DNNs and RNNs to performance levels that were achieved before only with Hessian-Free optimization \cite{SGD_2013}.

 %OU ESSE!

 The Adagrad optimizer comes from a family of subgradient methods that dynamically incorporate the concept of the previously observed data geometry in interactions to realize learning based on more informative gradient. Metaphorically, the adaptation allows finding small things in a large field \cite{Adagard_2011}.

 %OU PODE AINDA SER ESSE

 The Nadam algorithm was developed to improve the performance of deep learning systems, using a first-order algorithm that is more powerful but more computationally demanding than the second-order algorithm \cite{Nadam_2016}.

 %E TERMINA COM ESSE PARAGRAFO
%%% Acho que não precisa deste parágrafo
 To conduct the experiments, we used the software "Compara Classificadores Tf2," which was made available by the Inovisão research group. The software was configured with the proposed D-CNN networks and the optimizers used in each one for the experiment.


 %EXPERIMENTAL DESIGN

The experiments involved training a D-CNN (Deep Convolutional Neural Network) to classify different morphological characteristics in pigs as either normal or abnormal. As mentioned before, one of the characteristics studied was a spot, which is not considered a health abnormality but rather a natural characteristic that can be confused with some abnormalities. There were a total of five experiments, each focusing on a different morphological characteristic. For each experiment, the dataset contained images of both normal and abnormal examples of that morphological characteristic. The goal of the D-CNN was to accurately classify each image as either normal or abnormal for that particular morphology. Overall, the objective of the experiments was to evaluate the performance of the D-CNN in accurately classifying different morphological characteristics in swine.

The neural networks were evaluated separately for each morphological characteristic.


%% Não precisa
%The procedure uses the same networks and THE optimizer (COLOCAR O NOME DO OTIMIZADOR QUE VAMOS USAR) for each experiment and the same set of hyper-parameters. This approach ensures that any differences in the results between experiments are primarily due to the variations in the data rather than any differences in the neural network or its optimization. By using this approach, the researchers can analyze the performance of the D-CNN networks in a consistent manner, and determine how well they can differentiate between normal and abnormal images of the studied morphology. This can provide insights into the effectiveness of the D-CNN approach for image classification tasks and may help to identify areas for further improvement. The hyper-parameters and their values are shown in table \ref{Table_4}.

  %TABELA 04 NÃO FOI ALTERADA - NÃO PRECISOU

  % O PARAGRAFO ABAIXO CONTINUA IGUAL - PELO MENOS

  To evaluate the performance of the algorithm in this article, precision, recall, and F-score are used as evaluation metrics. 
  
%% Não precisa desta parte
%These metrics are commonly used in classification tasks to measure the performance of a machine learning model. In summary, precision measures how well the model identifies positive instances, recall measures how well the model identifies all positive instances, and the F-score combines both metrics to provide an overall performance score.

  %A PARTE DOS BOXPLOTS CONTINUA IGUAL
% Não precisa explicar o que é um boxplot, só falar que geramos se usarmos na discussão dos resultados.
  %To compare the performance of different D-CNNs and optimizers on the morphology dataset studied, boxplots were used. Boxplots are a common visualization technique used to display the distribution of a dataset, including its median, quartiles, and outliers. In the context of machine learning, boxplots can be used to compare the performance of different models or algorithms on a given dataset. In this study, the metrics of Precision, Recall, and F-Score were plotted in the boxplots. By comparing the boxplots for different D-CNN and optimizer combinations, it is possible to identify which models and algorithms perform best on the morphology dataset studied. This can help to choose the best model and optimizer for future experiments or applications of the D-CNN.

  %A PARTE QUE FALA SOBRE A VALIDAÇÃO CRUZADA - NÃO MUDOU
% Não precisa explicar o que é validação cruzada, só falar que usou.
%%% Por que 5 dobras?
  %Cross-validation is a common technique used to evaluate the performance of a machine-learning model and to generalize it to new data. The dataset is randomly split into 5 groups or "folds", with each fold containing roughly the same number of samples. The model is then trained and tested 5 times, with a different fold used for testing in each iteration, and the remaining folds used for training. This ensures that every sample in the dataset is used for testing exactly once, and the overall performance of the model is averaged across the 5 iterations.

  %AQUI NO MEIO ESTA A PARTE QUE FALA SOBRE OS TESTES ESTATISTICOS - TEMOS Q REVISAR A QUESTÃO DO ANOVA RETIRAR O SHAPIRO WILK E INSERIR O SCOTT-KNOTT

  %FOI INSERIDO A PARTE SOBRE SCOTT-KNOTT TEST - TALVEZ INSERIR UM POUCO + DE INGFORMAÇÃO DO SCOTT - KNOTT

% Não precisa explicar o propósito da ANOVA, nem do teste de Scott-Knott, só falar que usou e o limiar de 5%
%The performance was evaluated using statistical concepts. ANOVA was used to determine whether there are significant differences between the means of the networks. In the context of machine learning, it can be used to compare the performance of different algorithms or models on a given dataset. The 5\% significance level means that you would reject the null hypothesis (that there is no significant difference between the groups) if the p-value is less than 0.05.
%Scott-Knott test is a statistical technique used to rank and compare different Artificial Intelligence (AI) algorithms based on their performance on a given task or dataset. The Scott-Knott test is useful for comparing multiple AI algorithms, as it allows researchers to identify which algorithms are statistically significantly different in terms of their performance, and can also help identify which algorithms may be better suited for specific tasks or datasets.   


  %%%A PARTE DO GRAD-CAM CONTINUA IGUAL - NÃO HÁ ALERAÇÃO
%% Só falar que usou
  %The Grad-CAM (Gradient-weighted Class Activation Mapping) tool was used to visualize the regions of an image that a deep convolutional neural network (D-CNN) focuses on during processing. This visualization technique can help explain how a D-CNN makes its predictions by highlighting the regions of an image that contribute the most to the final classification. Specifically, Grad-CAM uses the gradient information of the final convolutional layer of the network to generate a heat map that indicates the importance of each pixel in the input image for the predicted class. By visualizing the heat map generated by Grad-CAM, it is possible to identify the regions of an image that the network considers most important for its classification decision. This can be useful for understanding why the network made certain correct or incorrect predictions and for identifying potential weaknesses or biases in the model. Overall, using Grad-CAM can be a useful tool for gaining insights into the decision-making process of a D-CNN and for improving the interpretability and transparency of machine learning models \cite{Grad-Cam}.


  %%%%RESULTADOS

  %O PRIMEIRO PARAGRAFO FALA SOBRE OS BOX PLOTS - COMO VAMOS USAR UM UNICO OTIMIZADOR, VERIFICAR COMO CONSEGUIREMOS COLOCAR ESSAS INFORMAÇÕES EM UM UNICO GRAFICO - 

  %UM GRAFICO PARA PRECISÃO, OUTRO PARA RECALL E OUTRO PARA FSCORE

%EM CADA GRAFICO COLOCA AS 05 MORFOLOGIAS ALINHADAS NO GRAFICO DE CADA REDE

%ESSE É O PARAGRAFO ANTIGO:
%The figures \ref{fig: Box_Caudofagia}, \ref{fig: Box_Auricular}, \ref{fig: Box_Arranhados}, \ref{fig: Box_vermelhidão}, and \ref{fig: Box_Manchas} refer to the boxplots showing the performance of the D-CNN and optimizers, for the five experiments conducted on the five morphologies studied in this work. 

%FICARIA +- ASSIM:
%% Vamos pensar sobre a apresentação dos boxplots. Talvez fique melhor se fizermos três figuras, uma pra cada métrica, com cinco gráficos em cada uma, um pra cada anomalia, em vez de cinco figuras com três gráficos.
%% Se formos usar na discussão...
The figures \ref{a}, \ref{b}, and \ref{c} refer to the box plots showing the performance of Precision, Recall, and F-score for each D-CNN applied to the five morphologies studied in this paper.

%SOBRE O PARAGRAFO QUE FALA SOBRE AS TABELAS ESTATISTICAS O TEXTO ORIGINAL TEM 03 TABELAS, UM PARA CADA MÉTRICA, P, R & F.
%POREM OS DADOS NA PRIMEIRA VERSÃO DESSAS TABELAS FORAM SELECIONADOS ESCOLHENDO OS VALORES + ALTOS COM BASE NA REDE E NO OTMIZADOR, COMO AGORA O OTIMIZADOT VAMOS USAR SOMENTE 01, SOME UMA COLUNA - OPTMIZER  - E OS VALORES REPORTADOS SERÃO REFERENTE AO OTMIZADOR SELECIONADO.

% O TEXTO ORIGINAL É ESSE ABAIXO:
%CREIO Q NÃO PRECISA ALTERAR, NUM PRIMEIRO MOMENTO
%% Acho que pra apresentarmos as tabelas, já que vamos usar um otimizador só, dá pra pensar em apresentar os resultados pra todas as redes
The tables \ref{Estatistica_Precisao}, \ref{Estatistica_Recall}, and \ref{Estatistica_F1Score} show the precision, recall, and F1 score, respectively, for the networks that exhibited the highest performance for each analyzed morphology. The median, IQR, average, and standard deviation were used as the criteria for evaluating the performance of these metrics.

%JÁ EM RELAÇÃO AS TABELAS FICARIAM ASSIM: (TEM Q COLOCAR OS VALORES)

%PRECISÃO
\begin{table}[h!] %tem q inserir \begin{table} para funcionar a legenda 'caption'
\begin{center}
\caption{Performance statistics of algorithms that had high performance about Precision metric}
\label{Estatistica_Precisao_1}
    \begin{tabular}{|p{1,9cm}|p{1,9cm}|p{1,9cm}|p{1,9cm}|p{1,9cm}|p{1,9cm}|}
     \hline    
     Morphology  &  Network  & Median & IQR & Average & Standard Deviation  \\ [0.5ex]
     \hline
     \hline
     Caudophagy &        &    &     &     &   \\
     \hline
     Ear Hematoma &     &       &      &      &      \\
     \hline 
     Redness &      &      &      &        &      \\
     \hline
     Scratches &      &      &      &     &    \\
     \hline
     Spots &      &     &      &     &        \\
     \hline
     
    \end{tabular}
\end{center}
\end{table}


%RECALL

\begin{table}[h!] %tem q inserir \begin{table} para funcionar a legenda 'caption'
\begin{center}
\caption{Performance statistics of algorithms that had high performance about Recall metric}
\label{Estatistica_Recall_1}
    \begin{tabular}{|p{1,9cm}|p{1,9cm}|p{1,9cm}|p{1,9cm}|p{1,9cm}|p{1,9cm}|}
     \hline    
     Morphology  &  Network  & Median & IQR & Average & Standard Deviation  \\ [0.5ex]
     \hline
     \hline
     Caudophagy &     &     &      &     &    \\
     \hline
     Ear Hematoma &     &      &    &     &      \\
     \hline 
     Redness &    &     &    &    &     \\
     \hline
     Scratches &    &    &      &       &    \\
     \hline
     Spots &    &     &     &     &       \\
     \hline
     
    \end{tabular}
\end{center}
\end{table}


%FSCORE
\begin{table}[h!] %tem q inserir \begin{table} para funcionar a legenda 'caption'
\begin{center}
\caption{Performance statistics of algorithms that had high performance about Fscore metric}
\label{Estatistica_F1Score_1}
    \begin{tabular}{|p{1,9cm}|p{1,9cm}|p{1,9cm}|p{1,9cm}|p{1,9cm}|p{1,9cm}}
     \hline    
     Morphology  &  Network & Median & IQR & Average & Standard Deviation  \\ [0.5ex]
     \hline
     \hline
     Caudophagy &    &    &     &    &     \\
     \hline
     Ear Hematoma &    &     &    &     &     \\
     \hline 
     Redness &    &    &     &     &    \\
     \hline
     Scratches &     &    &     &     &     \\
     \hline
     Spots &    &    &     &     &      \\
     \hline
     
    \end{tabular}
\end{center}
\end{table}

%%%NA SEQUENCIA DO TEXTO TEM A TABELA QUE MOSTRA O VISUAL DO GRAD-CAM, EM UM PRIMEIRO MOMENTO NÃO PRECISA MEXER NELA, SÓ DEPOIS TALVEZ SUBSTITUIR AS IMAGENS DELA POR IMGS QUE CONTENHAM O OTIMIZADOR SELECIONADO - BUSCAR ELAS NAS PASTAS

%%%NA SEQUENCIA DA DISCUÇÃO VEM A PARTE QUE FALAVA SOBRE A ANOVA   

%O TEXTO ORIGINAL ESTA DESCRITO ASSIM:

%Regarding the statistical tests, the tables \ref{Anova_Morfologias} show the ANOVA results for the metrics Precision, Recall, and Fscore. The value of Pr.Fc represents the variable "p", and when it is less than 5\%, it can be concluded that there is a statistical difference between the groups' performance. When it is higher than 5\%, it means that there is no evidence of a statistical difference between the groups, in this case, between the algorithms and optimizers for each morphology evaluated.

%PRECISA VERIFICAR SE FAZ SENTIDO O DESCRITO ACIMA

%COMO OS VALORES DOS TESTES DE ANOVA, SHAPIRO-WILK (Q NÃO VAI + USAR) E SCOTT-KNOTT FORAM OBTIDOS RODANDO OS TESTES COM TODOS AS REDES E TODOS OS OTMIZADORES, NÃO TERIA Q AGORA RODAR SÓ COM O OTMIZADOR SELECIONADO PARA GERAR NOVAMENTE ESSES VALORES?

==> Tabelas_Gr__ficos_SGD.tex <==

%%%HEMATOMA AURICULAR

\begin{table}[h!] %tem q inserir \begin{table} para funcionar a legenda 'caption'
\begin{center}
\caption{Statistics Metrics for Hematoma Auricular}
\label{Statisitics_SGD_Auricular}
    \begin{tabular}{|p{1,9cm}|p{1,5cm}|p{1,5cm}|p{1,5cm}|p{1,5cm}|}
     \hline    
     Architecture &  Median  &  IQR & Mean & SD  \\ [0.5ex]
     \hline
     \hline
     Precision & - & - - & - \\
     \hline
     EfficientNet a & 0.74110 & 0.261350 & 0.76143 & 0.14168256    \\
     \hline
     Xception a & 0.77380 & 0.068425 & 0.74059 & 0.09274094  \\
     \hline 
     InceptionResNetV2 a & 0.77440 & 0.092575 & 0.71168 & 0.11654245  \\
     \hline
     InceptionV3 a & 0.68055 & 0.156875 & 0.71204 & 0.11334596  \\
     \hline
     DenseNet201 b & 0.65150 & 0.376775 & 0.62151 & 0.16888514 \\
     \hline
     MobileNetV2 b & 0.40245 & 0.498650 & 0.50813 & 0.13544400 \\
     \hline
     \hline
     Recall &  &  &  &  \\
     \hline
     EfficientNet a & 0.70465 & 0.238150 & 0.73617 & 0.14168256 \\
     \hline
     Xception a & 0.76785 & 0.127925 & 0.71827 & 0.09274094 \\
     \hline
     InceptionResNetV2 a & 0.72620 & 0.136925 & 0.70823 & 0.11654245  \\
     \hline
     InceptionV3 a & 0.65480 & 0.161250 & 0.70680 & 0.11334596 \\
     \hline
     DenseNet201 b & 0.64880 & 0.250000 & 0.63681 & 0.16888514 \\
     \hline
     MobileNetV2 b & 0.51785 & 0.066050 & 0.57166 & 0.13544400  \\
     \hline
     \hline
     Fscore &  &  &  &   \\
     \hline
     EfficientNet a & 0.70985 & 0.243000 & 0.73471 & 0.1446753  \\
     \hline
     Xception a & 0.76640 & 0.142000 & 0.69762 &  0.1240729  \\
     \hline
     InceptionV3 a & 0.64520 & 0.157450 & 0.70018 & 0.1150254    \\
     \hline
     InceptionResNetV2 a & 0.72705 & 0.137500 & 0.68262 & 0.1553486  \\
     \hline
     DenseNet201 b & 0.64830 & 0.321150 & 0.61648 & 0.1899573  \\
     \hline
     MobileNetV2 b & 0.40415 & 0.172075 & 0.48054 & 0.1871248  \\
     \hline
          
    \end{tabular}
\end{center}
\end{table}

%####INSERIR BOX PLOT AQUI ####

%### INSERIR MATRIZES DE CONFUSÃO

%#### INSERIR GRAD CAM?

%%% CAUDOFAGIA

\begin{table}[h!] %tem q inserir \begin{table} para funcionar a legenda 'caption'
\begin{center}
\caption{Statistics Metrics for Hematoma Auricular}
\label{Statisitics_SGD}
    \begin{tabular}{|p{1,9cm}|p{1,5cm}|p{1,5cm}|p{1,5cm}|p{1,5cm}|}
     \hline    
     Architecture &  Median  &  IQR & Mean & SD  \\ [0.5ex]
     \hline
     \hline
     Precision & - & - - & - \\
     \hline
     EfficientNet a & 0.78790 & 0.106250 & 0.77890 & 0.06529067 \\
     \hline
     Xception a & 0.81485 & 0.142350 & 0.79656 & 0.09848896  \\
     \hline
     DenseNet201 a & 0.62500 & 0.194175 & 0.68623 & 0.12222341  \\
     \hline
     InceptionResNetV2 a & 0.83750 & 0.096500 & 0.80627 & 0.11574013 \\
     \hline
     InceptionV3 a & 0.79220 & 0.027425 & 0.78794 & 0.08098734  \\
     \hline
     MobileNetV2 b & 0.47220 & 0.315750 & 0.52702 & 0.15154903  \\
     \hline
     \hline
     Recall &  &  &  &  \\
     \hline
     EfficientNet a & 0.77780 & 0.102275 & 0.76313 & 0.06529067  \\
     \hline
     Xception a & 0.80555 & 0.153975 & 0.79091 & 0.09848896  \\
     \hline
     DenseNet201 a & 0.61110 & 0.152725 & 0.66465 & 0.12222341  \\
     \hline
     InceptionResNetV2 a & 0.80555 & 0.153975 & 0.77171 & 0.11574013  \\
     \hline
     InceptionV3 a & 0.77780 & 0.133825 & 0.74193 & 0.08098734  \\
     \hline
     MobileNetV2 b & 0.47220 & 0.166700 & 0.52725 & 0.15154903  \\
     \hline
     \hline
     Fscore &  &  &  &   \\
     \hline
     EfficientNet a & 0.77200 & 0.104875 & 0.76011 & 0.06573887 \\
     \hline
     Xception a & 0.80390 & 0.151625 & 0.78901 &  0.09942117  \\
     \hline
     DenseNet201 a & 0.60495 & 0.153300 & 0.64525 & 0.14010736\\
     \hline
     InceptionResNetV2 a & 0.79950 & 0.158525 & 0.75805 & 0.13304709 \\
     \hline
     InceptionV3 a & 0.77500 & 0.145050 & 0.72548 & 0.10041984  \\
     \hline
     MobileNetV2 a & 0.45130 & 0.194400 & 0.48574 & 0.16659319 \\     
     \hline
          
    \end{tabular}
\end{center}
\end{table}


==> ajustes.tex <==
\newcommand{\nomeEditor}{Professor Spyros Fountas, PhD and Dr. Stephen Symons, PhD}
\newcommand{\nomeArtigo}{Using Deep Learning for Morphological Classification in Pigs with a Focus on Sanitary Monitoring}
\newcommand{\nomeRevista}{Smart Agricultural Technology}
\newcommand{\nomeAutor}{Eduardo Bedin}
